The flat tail in the burst energy distribution of FRB 20240114A

Fast Radio Bursts (FRBs) are enigmatic millisecond-duration radio transients of extra-galactic origin, whose underlying mechanisms and progenitors remain poorly understood. FRBs are broadly classified into two categories: repeating FRBs, which emit multiple bursts over time, and one-off FRBs, which are detected as single events. A central question in FRB research is whether these two classes share a common origin. In this study, we present observations of FRB 20240114A, a repeating FRB that entered a hyperactive phase in January 2024. We conducted a 318-hour monitoring campaign using the Kunming 40-Meter Radio Telescope (KM40M) in the S-band (2.187-2.311 GHz), during which we detected eight radio bursts. We analyzed their properties, including dispersion measure (DM), bandwidth, pulse width, flux, fluence, and energy. Additionally, we searched for counterparts in overlapping data from the Five-hundred-meter Aperture Spherical Telescope (FAST) in the L-band (1.0-1.5 GHz). While no bursts were temporally aligned between the two telescopes, we identified one FAST burst that arrived approximately 6 ms after one of the KM40M bursts. The absence of FAST counterparts for the KM40M bursts suggests that individual bursts from FRB 20240114A are likely narrow-band, with fractional bandwidths less than 10%. By comparing the cumulative event rates from KM40M and FAST observations, we found that the two measurements are compatible, indicating a possible flattening of the event rate at higher energies. This feature aligns with observations of one-off FRBs, supporting the hypothesis that repeating and one-off FRBs may share a common origin.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org


==> tab.tex <==
\begin{table}[t]
    \centering
    \caption{Radio bursts detected with KM40M \label{tab:FRB_KM40m}}
    \begin{tabular}{ccccccccc}
    \hline \hline
         \textbf{Burst index} &\textbf{TOA} & \textbf{BW} & \textbf{Width} & \textbf{Flux} & \textbf{Fluence} & \textbf{$E_{\rm iso}$} & \textbf{$\rm DM_{SNR}$}{*} & \textbf{$\rm DM_{opt}$}{\textdagger} \\
         &$\rm MJD$ & $\rm MHz$ & $\rm ms$ & $\rm Jy$ & $\rm Jy\cdot ms$ & $\rm 10^{39}\:erg$ & $\rm pc\cdot cm^{-3}$ & $\rm pc\cdot cm^{-3}$ \\
         \hline
         1& 60418.02105159 & 2208.0-2287.7 2290.7-2310.5 & $5.6_{-1.0}^{+1.0}$ & $100_{-50}^{+20}$ & $190_{-100}^{+40}$ & $8.3_{-4.0}^{+1.7}$ & $527.5_{-1.7}^{+2.1}$ & $528.9_{-3.1}^{+3.1}$ \\
         2& 60427.99986798 & 2223.4-2229.2 2231.2-2310.5 & $5.0_{-0.8}^{+0.8}$ & $60_{-12}^{+12}$  & $151_{-30}^{+30}$ & $5.5_{-1.1}^{+1.1}$ & $524.2_{-3.4}^{+2.3}$ & $527_{-13}^{+13}$ \\
         3& 60428.01759323 & 2225.2-2233.1 2271.8-2310.5 & $4.7_{-0.9}^{+0.9}$ & $91_{-18}^{+18}$  & $160_{-32}^{+32}$ & $3.2_{-0.6}^{+0.6}$ & $536_{-8}^{+8}$ & $526_{-9}^{+9}$ \\
         4& 60518.85123378 & 2199.2-2225.5 & $5.3_{-1.2}^{+1.2}$ & $170_{-80}^{+34}$ & $230_{-110}^{+50}$ & $2.6_{-1.3}^{+0.5}$ & $538.6_{-1.1}^{+1.1}$ & $560_{-90}^{+90}$ \\
         5& 60520.70816271 & 2189.5-2197.3 2200.2-2310.5 & $3.6_{-0.5}^{+0.5}$ & $210_{-100}^{+40}$ & $270_{-140}^{+50}$ & $13.8_{-7.0}^{+2.8}$ & $535.6_{-0.8}^{+0.9}$ & $530.8_{-1.5}^{+1.5}$ \\
         6& 60520.79281743 & 2213.9-2300.8 & $2.8_{-0.7}^{+0.7}$ & $57_{-28}^{+11}$ & $66_{-32}^{+13}$ & $2.4_{-1.2}^{+0.5}$ & $528_{-5}^{+5}$ & $527_{-13}^{+13}$ \\
         7& 60566.54379544 & 2189.5-2197.3 2200.2-2310.5 & $2.2_{-0.4}^{+0.4}$ & $104_{-50}^{+21}$ & $101_{-50}^{+20}$ & $5.1_{-2.5}^{+1.0}$ & $524.2_{-2.1}^{+1.6}$ & $527.6_{-2.8}^{+2.8}$ \\
         8& 60566.59313771 & 2200.2-2239.3 2247.1-2303.7 & $3.9_{-1.0}^{+1.0}$ & $46_{-23}^{+9}$ & $86_{-40}^{+17}$ & $3.5_{-1.7}^{+0.7}$ & $525.8_{-2.3}^{+2.7}$ & $527_{-8}^{+8}$ \\
    \hline \hline
    \end{tabular}
    \begin{tabular}{l}
    * $\rm DM_{\rm SN}$ is the DM derived by maximizing the S/N. \\
    \textdagger $\rm DM_{\rm opt}$ is the DM derived using Fourier domain phase gradient method
    \end{tabular}
\end{table}

\begin{table}[t]
    \centering
    \caption{Radio bursts of FRB 20240114A with FAST}
    \label{tab:FRB_KM40m}
    \begin{tabular}{cp{2cm}cccccc}
    \hline \hline
         \textbf{TOA} & \textbf{Freq} & \textbf{PW} & \textbf{Flux} & \textbf{Fluence} & \textbf{Energy} & $DM_{\rm SNR}$ & $DM_{\rm opt}$ \\
         $(\rm topocenter)$ & $(\rm MHz)$ & $(\rm ms)$ & $(\rm Jy)$ & $(\rm Jy\cdot ms)$ & $(\rm 10^{39}\:erg)$ & $(\rm pc\cdot cm^{-3})$ & $(\rm pc\cdot cm^{-3})$ \\
         \hline
         60566.5438019957 & 1019.6-1174.5 1178.4-1466.7 & $2.31_{-0.1}^{+0.1}$ & $1.02_{-0.2}^{+0.2}$ & $1.14_{-0.23}^{+0.23}$ & $0.21_{-0.04}^{+0.04}$ & $529.15_{-0.05}^{+0.19}$ & $528.63_{-0.04}^{+0.04}$ \\
    \hline \hline
    \end{tabular}
\end{table}
